When Diffusion Models Memorize: Inductive Biases in Probability Flow of Minimum-Norm Shallow Neural Nets

While diffusion models generate high-quality images via probability flow, the theoretical understanding of this process remains incomplete. A key question is when probability flow converges to training samples or more general points on the data manifold. We analyze this by studying the probability flow of shallow ReLU neural network denoisers trained with minimal $\ell^2$ norm. For intuition, we introduce a simpler score flow and show that for orthogonal datasets, both flows follow similar trajectories, converging to a training point or a sum of training points. However, early stopping by the diffusion time scheduler allows probability flow to reach more general manifold points. This reflects the tendency of diffusion models to both memorize training samples and generate novel points that combine aspects of multiple samples, motivating our study of such behavior in simplified settings. We extend these results to obtuse simplex data and, through simulations in the orthogonal case, confirm that probability flow converges to a training point, a sum of training points, or a manifold point. Moreover, memorization decreases when the number of training samples grows, as fewer samples accumulate near training points.

==> unmerged_sec4_5.tex <==

\section{The probability flow and the score flow of min-cost denoisers}\label{sec:The probabilty flow and the score flow of min-cost denoisers}
\cnote{We want to marge section 4 and 5 to one section with our main results. The main idea is to present the result of score flow as way to gain intuition about the probability flow since it is a specific case. We would like for each dataset to first present the theorem of the score flow and then the theorem of the probability flow. The main idea to emphasis is that we can not sample a general point on the manifold using score flow and when using a diffusion time scheduler in probability flow we can. I hope tomorrow I will have time to prove the result of probability flow for the case equilateral triangle.}
In this section, we consider the probability flow and the score flow for denoisers which are min-cost solutions. 
We first consider the case of orthogonal dataset.
Suppose we have $N$ training points $\{\bv x_n\}_{n=0}^{N-1}$ where $\bv x_0 =\bm 0$ and the remaining training points are orthogonal, i.e., $\bv x_i^\top \bv x_j = 0$ for all $i,j>0$ with $i\neq j$. \footnote{The result holds for the general case where $\bv x_0$ is non-zero, provided that $\left( \bv x_i-\bv x_0\right)^\top\left( \bv x_j-\bv x_0\right) = 0$.} Let $\vu_n = \vx_n/\|\vx_n\|$ for all $n=1,...,N-1$. A minimizer $\bv f^*$ is given by \citep[proof of Theorem 4]{zeno2023how}
\begin{align}
    \bv f^*_{\rho_t}(\bv y) = \sum_{n=1}^{N-1}  \frac{\left \Vert \bv x_n \right \Vert}{\left \Vert \bv x_n \right \Vert-2\rho_t} \left([\vu_n^\top \vy-\rho_t]_+ + [\vu_n^\top \vy-\left(\left \Vert \bv x_n \right \Vert-\rho_t\right)]_+ \right)\vu_n.\label{eq:orthogonal_minimizer}
\end{align}

For small noise levels (i.e., for all $\min_{n\in[N-1]}\frac{\rho_t}{\left \Vert \bv x_n \right \Vert} \ll 1$) we can use Taylor's approximation to obtain the following score estimation 
\begin{align}
    \bv s_{\theta}\left(\bv y,t\right) =\frac{1}{\sigma_t^2} \left(\sum_{n=1}^{N-1} \bv u_n  \phi(\bv u_n^{\top} \bv y) - \left(\bv I - \sum_{n=1}^{N-1} \bv u_n \bv u_n^{\top}\right)\bv y\right)
     \label{eq:score estimation orthogonal}
\end{align}
where 
\begin{align}
    \phi(z) = \begin{cases} 
    -z & z < \rho_t \\
    \rho_t\left(\frac{2}{\left\Vert \bv x_n\right\Vert} z -1\right) & \rho_t < z < \left\Vert \bv x_n\right\Vert - \rho_t \\
    \left\Vert \bv x_n\right\Vert  - z & z > \left\Vert \bv x_n\right\Vert - \rho_t
    \end{cases}\,.
\end{align}


\begin{theorem} \label{theorem: orthogonal probability flow convergence}
Suppose that we have $N$ training points $\{\bv x_n\}_{n=0}^{N-1}$ where $\bv x_0 = \bm 0$ and $\bv x_i^\top \bv x_j = 0$ for all $i\ne j$. Given an initialization point $\bv y_T$, let $\mathcal{I}\subseteq [N-1]$ such that $|\mathcal{I}|\ge 2$ and $\rho_T < \bv u_i^\top \bv y_T  < \left \Vert \bv x_i \right \Vert-\rho_T$ for all $i\in\mathcal{I}$ and either $ \bv u_j^\top \bv y_T  < \rho_T$ or $ \bv u_j^\top \bv y_T > \left \Vert \bv x_i \right \Vert-\rho_T$ for all $j\in [N-1]\setminus\mathcal{I}$. Consider the probability flow 
\begin{align}
    \frac{\mathrm{d} \bv y_t}{\mathrm{d}t}=-\sigma_t \frac{\mathrm{d} \sigma_t}{\mathrm{d}t}\nabla\log p\left(\bv y_t,\sigma_t\right)
\end{align}
where $\sigma_t=\sqrt{t}$ and we estimate the score using \eqref{eq:score estimation orthogonal}.
Then we converge to a point on closest face of the hypercube to the initialization point $\bv y_T$ if $T > \tau_1$
and if  $T > \tau_2$ we converge to the closest point in the set $\mathcal{A} = \{ \sum_{n \in \mathcal{I}} \bv x_n \mid  \mathcal{I} \subseteq [N-1] \}$ to the initialization point $\bv y_T$. 
\end{theorem}
See Appendix \ref{Appendix: proof orthogonal probability flow convergence} for the proof. Note that if $\mathcal{I}$ is an empty set we always converge to the closest point in the set $\mathcal{A}$ to the initialization $\bv y_{T}$. Theorem \ref{theorem: orthogonal probability flow convergence} shows that the probability flow converges to a vertex of the hypercube or a point on the face of the hypercube. We consider this hypercube as an implicit data manifold. Note that we do not assume an explicit sampling model, such as a distribution supported on the manifold. 

This result aligns well with empirical findings that diffusion models can memorize individual training examples and generate them during sampling \citep{carlini2023extracting}. Additionally, \cite{duan2023are} showed that training data tend to have lower estimation errors (MSE) compared to hold-out samples, enabling the precise identification of training data with high confidence. In addition, an empirical result shows that Stable Diffusion can reproduce training data by piecing together foreground and background objects that it has memorized \citep{somepalli2023diffusion}. This behavior resembles our result on the sum of training points. In Stable Diffusion, we observe a ``semantic sum'' of training points, however,  our analysis focuses on the probability flow of a simple 1-hidden-layer model, while in practice, deep neural networks are capable of resulting more intricate semantic summations.

Next, we generalize Theorem \ref{theorem: orthogonal probability flow convergence} to a non-orthogonal training set.
Suppose the convex hull of the training points $\{\vx_1,\vx_2,...,\vx_{N}\} \subset \R^d$ is a $(N-1)$-simplex such that $\vx_1$ forms an obtuse angle with all other vertices.  Let $\vu_n = \vx_n/\|\vx_n\|$ for all $n=1,...,N-1$. The minimizer $\bv f^*$ is given by 
\begin{align}
    \bv f^*_{\rho_t}\left(\bv y\right)=\sum_{n=2}^{N} \frac{\left \Vert \bv x_n \right \Vert}{\left \Vert \bv x_n \right \Vert -2 \rho_t}  \left([\bv u_n^\top \bv y - \rho_t]_+ -[\bv u_n^\top \bv y - \left(\left \Vert \bv x_n \right \Vert -\rho_t\right)]_+\right)\bv u_n\,.
\end{align}
We assume  an initial point $\bv y_T$ such that $\rho_T <\bv u_i^\top \bv y_T < \left \Vert \bv x_i \right \Vert -\rho_T$ and $\bv u_j^\top \bv y_T < \rho$ for all $j \ne i$.
For small noise level (i.e. for all $i\in [N-1]$ $\frac{\rho_t}{\left \Vert \bv x_n \right \Vert} \ll 1$) we can use Taylor's approximation and obtain the following score estimation at a point $\bv y$ such that $\rho_t <\bv u_i^\top \bv y < \left \Vert \bv x_i \right \Vert -\rho_t$ and $\bv u_j^\top \bv y < \rho_t$ for all $j \ne i$ is
\begin{align}
    \bv s_{\theta}\left(\bv y,t\right) =\left(\left(1+\frac{2}{\left\Vert \bv x_{i}\right\Vert }\rho_t\right)\bv u_i \bv  u_i^{\top} -\bv I\right)\bv y - \rho_t\bv u_i \label{eq:score estimation obtuse}
\end{align}
\begin{theorem}\label{theorem: obtuse probability flow convergence}
Suppose the convex hull of the training points $\{\vx_1,\vx_2,...,\vx_{N}\} \subset \R^d$ is a $(N-1)$-simplex such that $\vx_1$ forms an obtuse angle with all other vertices. Given an initial point $\bv y_T$ such that $\rho_T <\bv u_i^\top \bv y_T < \left \Vert \bv x_i \right \Vert -\rho_T$ and $\bv u_j^\top \bv y_T < \rho_T$ for all $j \ne i$.
Consider the probability flow 
\begin{align}
    \frac{\mathrm{d} \bv y_t}{\mathrm{d}t}=-\sigma_t \frac{\mathrm{d} \sigma_t}{\mathrm{d}t}\nabla\log p\left(\bv y_t,\sigma_t\right)
\end{align}
where $\sigma_t=\sqrt{t}$ and we estimate the score using \eqref{eq:score estimation obtuse}.
Then we converge to a point on the line connecting $\bv x_1$ and $\bv x_i$ if $T < \tau$
and if  $T \ge \tau$ we converge to the closest point in the set $\{\bv x_1, \bv x_i\}$ to the initialization point $\bv y_T$.
\end{theorem}
See Appendix \ref{Appendix: proof obtuse probability flow convergence} for the proof.  Theorem \ref{theorem: obtuse probability flow convergence} shows that the probability flow converges to a point on the ray or to one of the edges of the ray. In this scenario, we consider the rays as the implicit data manifold.


\section{The score flow of min-cost denoisers}\label{sec:The score flow of min-cost denoisers}

To better understand the effect of the diffusion time scheduler $\sigma_t$, we analyze the score flow for denoisers that are min-cost solutions in this section.
For this dynamics, the stability condition for a stationary point  $\bv y$ is that any eigenvalue of the Jacobian matrix of the score function with respect to the input $\bv y$, i.e.,  $\lambda\left(\bv J\left(\bv y\right)\right)$ satisfies
\begin{align}
    \mathrm{Re}\{\lambda\left(\bv J\left(\bv y\right)\right)\}<0 \,. \label{eq:stability condition}
\end{align}
The following observation shows that in any model that perfectly fits an open ball of radius 
$\rho>0$ around the training point (and thus also interpolates the training set), the clean data points are stable stationary points of the score flow. This implies that, when initialized near these points, the process can converge to the clean data points.
\begin{proposition}
Let $\rho>0$ be arbitrary. 
Let $\bv f\left(\bv y\right)$ be a denoiser which satisfies  ${\bv f}(B(\vx_n,\rho)) = \{\vx_n\}$ for all $ n\in [N]$ (and thus interpolates the training data).  Then, any training point $\bv y \in \{\bv x_n\}_{n=1}^{N}$ is a stable stationary point of  \eqref{eq:score_flow} where we estimate the score using $s_{\bs \theta}\left(\bv y\right) = \frac{f(\vy)-\bv y}{\sigma^2}$.
\end{proposition}
\begin{proof}
For all $\bv y \in \{\bv x_n\}_{n=1}^{N}$ we get that $s_{\bs \theta}\left(\bv y\right) = 0$ since the denoiser interpolate the training data. In addition, for all $\bv y \in \mathrm{int}\left(B(\vx_n,\rho))\right)$ the Jacobian matrix is
\begin{align}
    \bv J\left(\bv y\right) = -\frac{1}{\sigma^2}\bv I\,,
\end{align}
therefore the stability condition \eqref{eq:stability condition} holds.
\end{proof}
This result aligns well with what we expect from the denoiser's prior distribution, as the training points should have high probability.

Next, we analyze the score flow. To gain intuition, we start with the case of orthogonal dataset.
We prove that the set of stationary points is the set of all possible sum of the training points.
\begin{theorem} 
Suppose that the training points $\{\bv x_0, \bv x_1,\bv x_2,...,\bv x_{N-1}\} \subset \R^d$ are orthogonal, i.e., for all $i\ne j$ $\bv x_i^\top \bv x_j = 0$ and $\bv x_0 = 0$. Then  the set of the stable stationary points of \eqref{eq:score_flow} is
$\mathcal{A} = \{ \sum_{n \in \mathcal{I}} \bv x_n \mid  \mathcal{I} \subseteq [N-1] \}$.
\end{theorem}
See Appendix \ref{appendix:proof orthogonal of stationary points} for the proof. 

Next, we prove that, given an initialization sufficiently close to the face of the hypercube where the stationary points correspond to the vertex coordinates, the dynamics converge to the face of the hypercube and then to a specific vertex.
\begin{theorem}\label{theorem: orthogonal score flow convergence}
Suppose that we have $N$ training points $\{\bv x_n\}_{n=0}^{N-1}$ where $\bv x_0 = \bm 0$ and $\bv x_i^\top \bv x_j = 0$ for all $i\ne j$. Given an initialization point $\bv y_0$, let $\mathcal{I}\subseteq [N-1]$ be the nonempty subset such that $\rho < \bv u_i^\top \bv y_0  < \left \Vert \bv x_i \right \Vert-\rho$ for all $i\in\mathcal{I}$ and either $ \bv u_j^\top \bv y_0  < \rho$ or $ \bv u_j^\top \bv y_0 > \left \Vert \bv x_i \right \Vert-\rho$ for all $j\in [N-1]\setminus\mathcal{I}$. Consider the score flow 
\begin{align}
    \frac{\mathrm{d}\bv y_t}{\mathrm{d}t} = \nabla \log p\left(\bv y\right)\,,
\end{align}
where we estimate the score using $\bs s_\theta\left(\bv y\right) = \frac{\bv f^*(\vy)-\bv y}{\sigma^2}$.
Then we converge to the nearest point from the set $\mathcal{A} = \{ \sum_{n \in \mathcal{I}} \bv x_n \mid  \mathcal{I} \subseteq [N-1] \}$ to the initialization point $\bv y_{T}$. In addition, for all $0 < \epsilon < \min_{i\in[N-1]}\left(\bv y_0\right)_i$ exists $\rho_0\left(\epsilon\right)$ and $T_0, T_1$ such that for all $\rho < \rho_0\left(\epsilon\right)$ the point $\bv y_T$ is not a stable stationary point and at most at distance $\epsilon$ from the face of the hypercube.
\end{theorem}
See Appendix \ref{appendix:proof orthogonal score flow convergence} for the proof. 

Next, we generalize the results for the case of an orthogonal dataset to more complex cases, including an obtuse simplex and equilateral triangle.
In the case of an obtuse simplex (Proposition \ref{prop:obtuse_triangle})  \nnote{incomplete sentence}
\begin{figure}[t]
	\centering
    \begin{subfigure}{0.5\linewidth}
    \centering
	   \includegraphics[width=\linewidth]{figures/score_obtuse_normalized.pdf}
        \caption{}
    \end{subfigure}%
	\begin{subfigure}{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/score_acute_normalized.pdf}
        \caption{}
    \end{subfigure}
	\caption{\textbf{The normalized score function of obtuse and acute simplex}. The red dots are the training points $\bv x_1, \bv x_2, \bv x_3$. The black lines are the ReLU boundaries. The score function is multiplied by the log of the norm of the score and divided by the norm of the score. In Figure (a) we plot the score function of an obtuse triangle. In Figure (b) we plot an equilateral triangle. }
 \label{fig:normalized score flow}
\end{figure}

In Figure \ref{fig:normalized score flow}, we illustrate the normalized score flow for the case of an obtuse $2$-simplex (see Figure \ref{fig:score flow} in Appendix \ref{appenix:Additional simulations} for the unnormalized score flow). As shown, the training points are stationary points. We prove that, in the general case of $N$ training points, the set of stable stationary points is a subset of the set of all partial sums of the training points. Additionally, we demonstrate that when the angles between data points are nearly orthogonal, a stable stationary point corresponding to the sum of the points exists.
\begin{theorem} \label{theorem:obtuse stationary points}
Suppose the convex hull of the training points $\{\vx_1,\vx_2,...,\vx_{N}\} \subset \R^d$ is a $(N-1)$-simplex such that $\vx_1$ forms an obtuse angle with all other vertices and $\bv x_1 = 0$. Then,  
the set  $\mathcal{A}$ of the stable stationary points of \eqref{eq:score_flow} satisfies
$ \{\bv x_n\}_{n=1}^{N} \subseteq \mathcal{A} \subseteq \{ \sum_{n \in \mathcal{I}} \bv x_n \mid  \mathcal{I} \subseteq [N] \}$. 
In addition, the point $\sum_{n \in \mathcal{I}} \bv x_n $ where $ \mathcal{I} \subseteq [N]$ and $|\mathcal{I}| \ge 2$ if $1 \notin \mathcal{I}$ and $|\mathcal{I}| \ge 3$ if $1 \in \mathcal{I}$ is stable stationary point if $\min_{k\in\mathcal{I}}\left\{ \sum_{i\in\mathcal{I} \setminus \{k\}}\bv u_k^\top \bv u_i \left\Vert \bv x_i\right\Vert \right\} >-\rho$.
\end{theorem}

See Appendix \ref{appendix:proof obtuse of stationary points}  for the proof. Notice that the condition $\min_{k\in\mathcal{I}}\left\{ \sum_{i\in\mathcal{I} \setminus \{k\}}\bv u_k^\top \bv u_i \left\Vert \bv x_i\right\Vert \right\} >-\rho$ holds for almost orthogonal dataset (and $\rho>0$).

Next, we prove that in the general case with $N$ training points, for small noise levels (i.e., small $\rho$) and an initialization point close to the rays connecting the base point ($\bv x_1$) to each training point ($\bv x_n$), the score flow converges to a point along a ray connecting the base point and another training point and then to a edge of the ray ($\bv x_1$ or $\bv x_n$ depending on initialization).

\begin{theorem}\label{theorem: obtuse of score flow convergence}
Suppose the convex hull of the training points $\{\vx_1,\vx_2,...,\vx_{N}\} \subset \R^d$ is a $(N-1)$-simplex such that $\vx_1$ forms an obtuse angle with all other vertices. Given an initial point $\bv y_0$ such that $\rho <\bv u_i^\top \bv y_0 < \left \Vert \bv x_i \right \Vert -\rho$ and $\bv u_j^\top \bv y_0 < \rho$ for all $j \ne i$, consider the score flow 
\begin{align}
    \frac{\mathrm{d}\bv y_t}{\mathrm{d}t} = \nabla \log p\left(\bv y\right)\,,
\end{align}
where we estimate the score using $\bs s_\theta\left(\bv y\right) = \frac{\bv f^*(\vy)-\bv y}{\sigma^2}$.
Then we converge to the closest edge of the ray. In addition, for all $0 < \epsilon < \bv u_i^\top \bv y_0$ exists $\rho_0\left(\epsilon\right)$ and $T_0, T_1$ such that for all $\rho < \rho_0\left(\epsilon\right)$ the point $\bv y_T$ is not a stable stationary point and at most at distance $\epsilon$ from the line between $\bv x_1$ and $\bv x_i$ for $T_0<T<T_1$.
\end{theorem}
See Appendix \ref{appendix:proof obtuse of score flow convergence}  for the proof.

In the case where the training points forming the vertices of an equilateral triangle we prove that we converge to an edge of the triangle (the implicit data manifold) and then to the closest vertex, for small noise radius ($\rho$), and initialization point near the edge of the triangle. 
\begin{proposition}
\label{theorem: equilateral triangle score flow convergence}
Suppose the convex hull of the training points $\vx_1,\vx_2,\vx_3 \in \R^d$ is an equilateral triangle. Given an initial point $\bv y_0$ such that $i\in\{1,2\}-\frac{\left\Vert \bv x_i\right\Vert}{2}+\rho<\bv u_i^{\top}\bv y_0<\left\Vert \bv x_i\right\Vert -\rho$ and $\bv u_3^{\top}\bv y < - \frac{\left\Vert \bv x_3 \right\Vert}{2} + \rho$, consider the score flow 
\begin{align}
    \frac{\mathrm{d}\bv y_t}{\mathrm{d}t} = \nabla \log p\left(\bv y\right)\,,
\end{align}
where we estimate the score using $\bs s_\theta\left(\bv y\right) = \frac{\bv f^*(\vy)-\bv y}{\sigma^2}$.
Then we converge to the closest vertex to the initialization point. In addition, for all $0 < \epsilon < \left(\bv u_1 + \bv u_2\right)^\top\bv y_0 - \frac{\left\Vert \bv x\right\Vert}{2}$ there exists $\rho_0\left(\epsilon\right)$ and $T_0, T_1$ such that for all $\rho < \rho_0\left(\epsilon, T\right)$ the point $\bv y_T$ is not a stable stationary point and at most $\epsilon$ distance from the line between $\bv x_1$ and $\bv x_2$ for $T_0<T<T_1$.
\end{proposition}
